Heavy Traffic Joint Queue Length Distribution without Resource Pooling

This paper studies the heavy-traffic joint distribution of queue lengths in two stochastic processing networks (SPN), viz., an input-queued switch operating under the MaxWeight scheduling policy and a two-server parallel server system called the $\mathcal{N}$-system. These two systems serve as representatives of SPNs that do not satisfy the so-called Complete Resource Pooling (CRP) condition, and consequently exhibit a multidimensional State Space Collapse (SSC). Except in special cases, only mean queue lengths of such non-CRP systems is known in the literature. In this paper, we develop the Transform method to study the joint distribution of queue lengths in non-CRP systems. The key challenge is in solving an implicit functional equation involving the Laplace transform of the heavy-traffic limiting distribution. For the $\mathcal{N}$-system and a special case of an input-queued switch involving only three queues, we obtain the exact limiting heavy-traffic joint distribution in terms of a linear combination of two iid exponentials. For the general $n\times n$ input-queued switch that has $n^2$ queues, under a conjecture on uniqueness of the solution of the functional equation, we obtain an exact joint distribution of the heavy-traffic limiting queue-lengths in terms of a non-linear combination of $2n$ iid exponentials.

==> extras.tex <==

In order to prove Lemma \ref{lem: 3q_analytic}, we first show that all the moments of $\epsilon\q$ exists as $\epsilon \rightarrow 0$, for which, we first show that the Moment Generating Function (MGF) of each of the component of $\epsilon \q$ exists in an interval around zero. First, consider the quadratic Lyapunov function $\|\q\|^2$. Then, the drift is given by
\begin{align*}
    \EE[\Delta \|\q\|^2 |\q] &= \EE[\|\q + \mathbf a - \mathbf s + \mathbf u\|^2|\q] -\|\q\|^2\\
    &=\EE[\|\mathbf a - \mathbf s + \mathbf u\|^2|\q] + 2 \EE[\langle \q, \mathbf a - \mathbf s + \mathbf u\rangle|\q] \\
    &\stackrel{(a)}{\leq} 3a_{\max}^2 + 2 \langle \q, \boldsymbol \lambda \rangle - 2\max_{\mathbf s} \langle \q, \mathbf s \rangle\\
    & \stackrel{(b)}{\leq} 3a_{\max}^2 + 2 (1-\epsilon)\langle \q, \boldsymbol \nu \rangle -  2\langle \q, \boldsymbol \nu \rangle\\
    & = 3a_{\max}^2  - 2\epsilon  \langle \q, \boldsymbol \nu \rangle,\\
    &\stackrel{(c)}{\leq} 3a_{\max}^2  - 2\epsilon \nu_{\min} \|\q\|,
\end{align*}
where (a) follows because $|a_i-s_i+u_i|\leq a_{\max}$ for all $i$, and $\langle \q,\mathbf u\rangle =0$; (b) follows by using the definition of $\boldsymbol \lambda$, and $\boldsymbol \nu$ being convex combination of $(1,0,0)$ and $(0,1,1)$; and (c) follows as $\langle \q, \boldsymbol \nu \rangle \leq \nu_{\min} \langle \q, \mathbf 1 \rangle \leq \nu_{\min}\|\q\|$. Thus, by using convexity of $\|\cdot\|^2$, we have 
\begin{align*}
    \EE[\Delta \|\q\| |\q] \leq \frac{1}{2\|\q\|}  \EE[\Delta \|\q\|^2 |\q] \leq  \frac{3a_{\max}^2 }{2\|\q\|}  - 2\epsilon \nu_{\min} \leq -\epsilon \nu_{\min},
\end{align*}
where the last inequality follows when $\epsilon\|\q\| \geq \kappa:= \frac{3a_{\max}^2 }{4\nu_{\min}}$.
Further, by triangle inequality, we also have,
\begin{align*}
    |\Delta \|\q\| | \leq  \|\Delta \q\| \leq 3a_{\max}. 
\end{align*}
Thus, we have,
\begin{align*}
    \EE\big[ \Delta e^{\epsilon\theta \|\q\| }\big|\q\big] &= e^{\epsilon\theta \|\q\| } \EE\big[ e^{\epsilon\theta \Delta \|\q\| } -1 \big|\q\big]\\
    & \leq e^{\epsilon\theta \|\q\| } \EE\Big[ \epsilon\theta \Delta \|\q\| +  \epsilon^2\theta^2 (\Delta \|\q\|)^2 e^{\epsilon\theta \Delta \|\q\| } \big|\q\Big]\\
    & \leq e^{\epsilon\theta \|\q\| } \EE\Big[ \epsilon\theta \Delta \|\q\| +  \epsilon^2\theta^2 (\Delta \|\q\|)^2 e^{\epsilon\theta \Delta \|\q\| } \big|\q\Big]\\
\end{align*}
